HiFi-123: Towards High-fidelity One Image to 3D Content Generation

Recent advances in diffusion models have enabled 3D generation from a single image. However, current methods often produce suboptimal results for novel views, with blurred textures and deviations from the reference image, limiting their practical applications. In this paper, we introduce HiFi-123, a method designed for high-fidelity and multi-view consistent 3D generation. Our contributions are twofold: First, we propose a Reference-Guided Novel View Enhancement (RGNV) technique that significantly improves the fidelity of diffusion-based zero-shot novel view synthesis methods. Second, capitalizing on the RGNV, we present a novel Reference-Guided State Distillation (RGSD) loss. When incorporated into the optimization-based image-to-3D pipeline, our method significantly improves 3D generation quality, achieving state-of-the-art performance. Comprehensive evaluations demonstrate the effectiveness of our approach over existing methods, both qualitatively and quantitatively. Video results are available on the project page.

==> images_tex/SDEdit.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.\textwidth]{images/ablate_sdedit.pdf}
  \caption{Novel view enhancement results of SDEdit.}
  % \vspace{-1em}
\label{fig:sdedit}
\end{figure}

==> images_tex/comp_syncdreamer.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.95\textwidth]{images/syncdreamer.pdf}
  \caption{Qualitative comparison with Syncdreamer. It can be found that our method can generate novel views with higher fidelity according to the reference image.}
  % \vspace{-1em}
\label{fig:comp_sync}
\end{figure}

==> images_tex/i23_gso.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=.9\textwidth]{images/i23_gso.pdf}
  \caption{Qualitative comparison with image-to-3D generation baselines on GSO dataset.}
  % \vspace{-1em}
\label{fig:i23_gso}
\end{figure}

==> images_tex/inversion_example.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.\textwidth]{images/inversion_example.pdf}
  \caption{Comparison between depth-based DDIM inversion and other inversion approaches.} 
  % \vspace{-1em}
\label{fig:ddim}
\end{figure}

==> images_tex/timestep.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.\textwidth]{images/timesteps.pdf}
  \caption{Ablation on time steps}
  % \vspace{-1em}
\label{fig:timestep}
\end{figure}

==> tables/algo.tex <==
\begin{algorithm}[tb]
\caption{RGSD loss}
\label{alg:rgsd}
\textbf{Input: }{Depth-conditioned SD model~\cite{SDD} $\epsilon_\phi$, reference image, 3D model with parameter $\theta$, attention injection start step $t=l$, learning rate $\eta$. }

\begin{algorithmic}[1]
% \STATE {\bfseries initialize} $n$ 3D structures $\{\theta^{(i)}\}_{i=1}^{n}$, a noise prediction model $\mathbf{\epsilon}_{\phi}$ parameterized by $\phi$.
\WHILE{not converged}
\STATE Sample camera pose $c$ and render $\bm{x}_0 = g(\theta,c)$
\STATE Sample time step $t = \tau$
\STATE\COMMENT{DDIM inversion}
\FOR{$t=1,2,...,l$} 
\STATE $\bm{x}_{t} = (\alpha_{t}/\alpha_{t-1})(\bm{x}_{t-1}-\sigma_{t-1}\epsilon_\phi)+\sigma_{t}\epsilon_\phi$ 
\ENDFOR
\STATE\COMMENT{DDIM sampling with attention injection}
\FOR{$t=l,l-1,...,\tau+1$} 
\STATE $\Tilde{\bm{x}}_{t-1} = (\alpha_{t-1}/\alpha_t)(\Tilde{\bm{x}}_t-\sigma_t\Tilde{\epsilon}_t)+\sigma_{t-1}\Tilde{\epsilon}_t$
\ENDFOR
\STATE Get enhanced state $\Tilde{\bm{x}}_\tau$, noise $\Tilde{\epsilon}_\tau$
\STATE Construct $\bm{x}_\tau = \alpha_\tau\bm{x}_0 + \sigma_\tau\Tilde{\epsilon}_\tau$
\STATE $\theta \leftarrow \theta - \eta\nabla_{\theta} \mathbb{E}[\|\bm {x}_\tau - \Tilde{\bm{x}}_\tau\|_2^2]$
\ENDWHILE
\STATE {\bfseries return} 
\end{algorithmic}
\end{algorithm}

==> tables/i23_gso.tex <==
\begin{table}[t]
\centering
    \resizebox{0.7\linewidth}{!}{
  \begin{tabular}{l|ccccc}
\toprule
 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & CD$\downarrow$ & IoU$\uparrow$\\ \midrule
Make-it-3D~\cite{tang2023make}& 22.38 & 0.734 & 0.251 & 0.086 & 0.368  \\
Magic123~\cite{qian2023magic123}& 30.16 & \textbf{0.789} & 0.237 & 0.066 & 0.461 \\
Ours& \textbf{32.05} & 0.785 & \textbf{0.221} & \textbf{0.055} & \textbf{0.493}\\
\bottomrule
\end{tabular}}
  \caption{Quantitative comparison with image-to-3D generation baselines on GSO dataset.}
  \label{tab:gso_i23}
  \vspace{-1.5em}
\end{table}

==> tables/i23_single.tex <==
%   \captionof{table}{Quantitative comparison with image-to-3D generation baselines.}
%   \label{tab:i23}
%   \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccc}
% \toprule
%  & LPIPS$\downarrow$  & Contextual$\downarrow$ & CLIP$\uparrow$ \\ \midrule
% RealFusion& 0.35 & 2.18& 0.81 \\
% Make-It-3D & 0.23 & 1.97& 0.90\\
% Magic123& \textbf{0.19} & 1.88 & 0.88  \\
% Ours& 0.21 & \textbf{1.63} & \textbf{0.92} \\
% \bottomrule
% \end{tabular}
%   }

\begin{table}[t]
\centering
  \resizebox{0.6\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
 & LPIPS$\downarrow$  & Contextual$\downarrow$ & CLIP$\uparrow$ \\ \midrule
RealFusion~\cite{melas2023realfusion}& 0.35 & 2.18& 0.81 \\
Make-It-3D~\cite{tang2023make} & 0.23 & 1.97& 0.90\\
Magic123~\cite{qian2023magic123}& \textbf{0.19} & 1.88 & 0.88  \\
Ours& 0.21 & \textbf{1.63} & \textbf{0.92} \\
\bottomrule
\end{tabular}}
  \caption{Quantitative comparison with image-to-3D generation baselines on single view dataset.}
  \label{tab:single_i23}
  \vspace{-1.5em}
\end{table}

==> tables/zero_metrics.tex <==
\setlength{\tabcolsep}{2pt}
\begin{figure}[t]
% \begin{minipage}[c]{0.470\linewidth}
%   \centering
%   \captionof{table}{Quantitative comparison with image-to-3D generation baselines.}
%   \label{tab:i23}
%   \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccc}
% \toprule
%  & LPIPS$\downarrow$  & Contextual$\downarrow$ & CLIP$\uparrow$ \\ \midrule
% RealFusion& 0.35 & 2.18& 0.81 \\
% Make-It-3D & 0.23 & 1.97& 0.90\\
% Magic123& \textbf{0.19} & 1.88 & 0.88  \\
% Ours& 0.21 & \textbf{1.63} & \textbf{0.92} \\
% \bottomrule
% \end{tabular}
%   }
% \end{minipage}\hfill
\begin{minipage}[c]{0.45\linewidth}
  \centering
  \resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
 & Contextual$\downarrow$ & CLIP$\uparrow$ \\ \midrule
Zero-1-to-3~\cite{liu2023zero}& 1.94 & 0.89  \\
Ours& \textbf{1.60} & \textbf{0.93} \\
\bottomrule
\end{tabular}}
  \captionof{table}{Quantitative comparison with Zero-1-to-3 on single view dataset.}
  \label{tab:zero_single}

\end{minipage}\hfill
\begin{minipage}[c]{0.5\linewidth}
  \centering
  \resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
 & PSNR$\uparrow$  & SSIM$\uparrow$ & LPIPS$\downarrow$ \\ \midrule
Zero-1-to-3~\cite{liu2023zero}& 34.58 & 0.763 & 0.231  \\
Ours& \textbf{36.89} & \textbf{0.795} & \textbf{0.214} \\
\bottomrule
\end{tabular}}
  \captionof{table}{Quantitative comparison with Zero-1-to-3 on GSO dataset.}
  \label{tab:zero_3D}

\end{minipage}\hfill
% \vspace{-1em}
\end{figure}
